Optimal Locally Repairable Codes with Improved Update Complexity

For a systematic erasure code, update complexity (UC) is defined as the maximum number of parity blocks needed to be changed when some information blocks are updated. Locally repairable codes (LRCs) have been recently proposed and used in real-world distributed storage systems. In this paper, update complexity for optimal LRC is studied and both lower and upper bounds on UC are established in terms of length (n), dimension (k), minimum distance (d), and locality (r) of the code, when (r+1)|n. Furthermore, a class of optimal LRCs with small UC is proposed. Our proposed LRCs could be of interest as they improve UC without sacrificing optimality of the code.

==> Sections/Comparison.tex <==
Our proposed optimal LRCs could achieve the lower bound on average UC in the case that there is only one information node update. In the following remark it is shown that our optimal LRCs have better UC in the case that any number of information node updates than other optimal LRCs, since our optimal LRCs have better $\overline{u_1}$. 
\begin{remark}
	In our proposed optimal LRCs, in the case that there are more than one information node updates, the average UC depends on the number of parity nodes connected to the updated information nodes in addition to number of edges in Tanner graph. However, if some information nodes are connected to the same parity nodes, average UC for those information nodes are depends on the number of edges between variable nodes and check nodes. Consequently, whenever we reach to the minimum average UC for one information update in our proposed optimal LRC, we minimized the number of edges as many as possible. Hence, by minimizing $\overline{u_1}$ in our proposed optimal LRC we also reduce $\{\overline{u_2}, \overline{u_3}, ...\}$ for the cases that there are more than one information updates which can be a minimum possible average UC.      
%	
%	In our proposed optimal LRCs, for average UC of one information node update, lower bound in \ref{modifiedbounduc} is achieved. For more than one information node update, except the number of parity nodes connected to each of the information nodes, it is important to find the parity nodes which are common between information nodes. Consequently, it could be possible that one code has better $\overline{u_1}$ than another code but it has the worst $\{\overline{u_2}, \overline{u_3}, ...\}$.    
\end{remark}

In order to evaluate UC of our proposed coding scheme, we compare our proposed $(n,k,d,r)=(15,9,5,4)$ optimal LRC presented in Example \ref{ex:ex} with one whose global check nodes are connected to $k+1$ variable nodes, which is the common approach in designing optimal LRCs (please see Fig. \ref{fig:3}).

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth, scale=0.5]{otheructan.pdf}
	\vspace{-.5 cm}
	\caption{Tanner graph of an $(n,k,d,r)=(15,9,5,4)$ optimal LRC. In this figure, each of the global check node are connected to $k+1=10$ variable nodes.}
	\vspace{-.4 cm}
	\label{fig:3}
\end{figure} 

The average UC associated with each LRC is computed when $1$ and $2$ information nodes update. 
In the following equations, we denote the average UC of our proposed LRC and that of other LRC by $\overline{u_x}^{LRC_1}$ and $\overline{u_x}^{LRC_2}$, respectively.
For $u_1$, we have 
\begin{multline*}
~~~~~~~~~~~~~~~~~~~~~~~~~ 4\le {u_{1}}\le 5 \\
~~~~\overline{u_{1}}^{LRC1}=\frac{9(d-1)}{9}=d-1=4\\
\overline{u_{1}}^{LRC2}=\frac{(d-1)+8d}{9}=d-0.11=4.89~~~~~~
\end{multline*} 
Similarly, for $u_2$, we have 
\begin{multline*}
~~~~~~~~~~~~~~~~~~~~~~~~~5\le {u_{2}}\le 6 \\
\overline{u_{2}}^{LRC1}=(26\times 5 + 10 \times 6)/{9\choose 2}=5.27\\
\overline{u_{2}}^{LRC2}=(20\times 5 + 16 \times 6)/{9\choose 2}=5.44~~~~~~~~
\end{multline*} 
Hence, our proposed optimal LRC suggests UC close to the lower bound obtained in Proposition \ref{prop:UCbound}. 
In this case, our proposed optimal LRC improves the UC by 18.2\% and 3.1\% for $\overline{u_1}$ and $\overline{u_2}$, respectively. 
Comparing with the general approach of designing optimal LRCs, this improvement is obtained without sacrificing other important properties of LRCs.

%In the following table we compare the general approach of code design and our proposed algorithm for some codes used in data storages.
%
%~~~~~~~~~~~.
%\begin{tabular}{|c|c|c|}
%	\hline \begin{tabular}{@{}c@{}}Name and parameters \\ $(n,k,d,r)$ of code\end{tabular}  &  \begin{tabular}{@{}c@{}} $\overline{u_1}$ for general \\ approach \end{tabular} &  \begin{tabular}{@{}c@{}} $\overline{u_1}$ for our \\ approach \end{tabular} \\ 
%	\hline Google $(9,6,4,6)$ & 4 & 4 \\ 
%	\hline Microsoft $(16,12,4,6.75)$ & 4 & 3.396 \\ 
%	\hline Facebook $(16,10,5,5)$ & 5 & 4.8 \\ 
%	\hline 
%\end{tabular}

%The difference between UC of our optimal LRCs and other LRCs is more in big sized LRCs. 
%For any number of information node updates in LRCs there is a different bound for UC and for any number of information node updates the average UC in our LRC is closer to the lower bound than other LRCs.     

==> Sections/Introduction__Mostafa_Shahabinejad_s_conflicted_copy_2016-04-11_.tex <==
%$\bullet$ Benefits of Distributed Storage Systems (DSS)
Distributed Storage Systems (DSSs) are common way for storing large scale data. DSS uses many storage nodes to store data and as a result data is stored in more than one node. Thus, it is a secure and reliable way to store data. In such systems, node failure is a common problem and it is caused by some reasons such as, physical problems and unavailability due to server maintenance. Therefore, in order to recover the lost data we need to add some redundant data such as data replication in storage nodes.
%However, providing too many storage nodes is not efficient due to their costs and maintenance.         

%$\bullet$ Challenges in DSSs

%$\bullet$ Benefits of erasure codes in DSSs

Replication of data is a costly method in order to add redundant data, thus recently erasure codes have been used in DSS to decrease storage overhead and make it efficient. At first step of erasure codes, the stripe of data is split into $k$ blocks and then these blocks code to $n$ blocks and store in $n$ different storage nodes. For a erasure code $(n,k)$ with minimum distance $d$, where $d \le n-k+1$, the $n - k$ additive nodes should be generated such that any $k$ node failure could be recovered by $n - d + 1$ nodes. Recently, erasure codes are being deployed in many cloud storage services such as Google Drive, Microsoft Azure and Facebook.     

%$\bullet$ Existing Solutions (1. regenerating codes, 2. Codes with disk I/O) 3. LRCs
Although erasure codes reduce storage overhead, they need access to many nodes to recover a failed node. For example, in a Maximum Distance Separable (MDS) $(n,k)$ code with minimum distance $d=n-k+1$, $K$ nodes should be used to recover one failure.    
%require high repair bandwidth, disk I/O, and computation. Therefore, regenerating codes, low disk I/O codes, and LRC codes have been proposed, to reduce repair bandwidth, disk I/O, and code locality, respectively.

%Repair bandwidth is defined as the amount of download required to recover a failed node and is one of the important factors in erasure codes which should be reduced. Reducing repair bandwidth needs increasing storage overhead, and there is a bound between them, proposed in [] to choose the efficient values. Regenerating codes are class of codes which are formed based on reducing the repair bandwidth in which each block of data is divided to some sub-blocks and to reconstruct the failed data only some sub-blocks of other nodes need to be download and as a result the repair bandwidth will be decreased.   

%Disk I/O, which is number of reads required for reconstruction failed node, also considered as a criterion to evaluate the efficiency of code, so, many codes have been proposed to deal with it such as []. 

The number of nodes required to recover a failed node is defined as a locality of code and denoted $r$. Locally repairable codes (LRCs) are a class of codes which their main concentration is on decreasing the number of participating nodes in recovery of a failed node. Increasing the locality of code needs high storage overhead so, this trade-off between locality and storage overhead should be considered to obtain optimal LRC. To achieve the optimal LRC there is a bound proposed in [], [] which make a connection between minimum distance and locality of codes. 
\begin{equation}\label{eq:minimumdistancebound} 
d \le n - k - \frac{k}{r} + 2
\end{equation}
%$\bullet$ Existing solution in LRCs (optimal LRCs)
Based the bound (\ref{eq:minimumdistancebound}) reducing locality, results in low minimum distance and so, will not be reliable anymore. However, increasing reliability needs high minimum distance which is $d = n - k + 1$ at maximum, which leads to worst locality which is $r=k$. As a result, the optimal LRC codes which follow this bound have the smallest locality and also maximum possible minimum distance in order to have appropriate reliability.    

%$\bullet$ Tuye LRCs ye seri local parity CNs va Global Parity CNs
%Globala b hame vaslan k sharte $d$ satisfy.  
%Global noda mitunan b ye ede vasl nabashan...
%Update complexity

%In order to visualize an $(n,k)$ linear block code we use tanner graph. All nodes in tanner graph are divided to two set, one set is consist of $n$ variable nodes and another set is $n-k$ parity check nodes (CNs). Parity check nodes in LRC codes are split to some local parity check nodes and some global check nodes as well. We assume that $r+1|n$, so in order to satisfy locality $r$ we divide variable nodes to ${\frac{n}{r+1}}$ groups and for each group we assign a local parity CN and attach all the group members to it. Furthermore, due to minimum distance $d$, global CNs which are $d-2$ nodes, should cover all variable nodes. In order to satisfy minimum distance $d$ there is no need to connect all variable nodes to all $d-2$ global parity CNs and we could connect each global parity CN to some variable nodes but also cover all $n$ variable nodes. By, reducing the number of edges between global CNs and variable nodes we are able to decrease complexity of code. 

As an example of $(n,k,r,d)$ LRC, two $(8,4,3,4)$ with different formation are shown in the figure $(1.a)$ and $(1.b)$. In the code $(a)$ global parity check nodes are connected to all variable nodes but in code $(b)$ are connected to only some variable nodes. Due to the connected edges, in the code $(a)$ all the shaded nodes depend on all $4$ systematic nodes. However, in the code $(b)$, $a_{1}$ depends on $\{1,2,3\}$, $a_{2}$ depends on $\{1,2,4\}$, $a_{3}$ depends on $\{2,3,4\}$, and $a_{4}$ depends on all $4$ systematic nodes. Therefore, in the code $(a)$, whenever each systematic node is updated, all the shaded nodes must be updated. On the other hand, in the code $(b)$ whenever node $\{1,3,4\}$ are updated, $3$ shaded nodes must be updated but for updating node $\{2\}$ all the shaded nodes must be updated. Thus, to update each systematic node in code $(a)$, $5$ nodes are updated but in code $(b)$, whenever node $\{1,3,4\}$ are updated, $4$ nodes must be updated and for node $\{2\}$, $5$ nodes should be updated. Moreover, the related equation of node $\{a_{2},a_{3}\}$ in both codes, are shown in $(2)$ and $(3)$. The number of appeared systematic nodes in these equations shows the complexity of these codes.            

\begin{figure}[t!]\label{fig:1}
	\graphicspath{ {Figures/} }
	\centering
	\includegraphics[width=0.5\textwidth, scale=0.5]{8434.pdf}
	\vspace{-.5 cm}
	\caption\small{Tanner graph of a $(8,4,3,4)$ with two different formation.}
	\vspace{-.4 cm}
	\label{fig:MarkovChain}
\end{figure}
\vspace{-.5 cm}
\begin{equation}\label{eq:uc1} 
a_{2}= x_{1}+x_{2}+x_{3}+x_{4} ~~~~~,~~~~~ a_{3}= x_{1}+x_{2}+x_{3}+x_{4}
\end{equation}
\vspace{-.4 cm}
\begin{equation}\label{eq:uc2} 
a_{2}= x_{1}+x_{2}+x_{4} ~~~~~,~~~~~ a_{3}= x_{2}+x_{3}+x_{4}
\end{equation}

%$\bullet$ Chera Update complexity...(definition)
The improvement in the number of updated nodes in code $(b)$ is obtained by reducing the edges of Tanner graph. Reducing the edges, leads to minimum dependency between variable nodes and so, whenever we need to update a variable node we could update only some nodes. So, Update complexity (UC) is defined as the number of nodes need to be updated, whenever we update one systematic node. In many applications such as cloud storage services, updating data is common and storage servers are updated frequently. So, it should be considered as a important factor in code design. 

%$\bullet$ Our Contribution(Bound, codes that achieve the bound...)
In this paper, we propose a bound for UC of LRCs, for each number of node update. Based on the proposed bound we design a class of codes that could achieve to the UC which is close to the lower bound. We also prove that this codes could have a good performance in updating any number of node update.   

%Organization of the paper:
The remainder of this paper is organized as follows. In Sec. II we provide required preliminaries. Then in Sec. III we introduce our proposed LRC to have efficient UC. Finally in Sec. IV we conclude the paper.   

% $k=\log_2(52)\times \frac{8}{7} + \gamma \xi\upsilon$

%\begin{equation}\label{eq:hadi} 
%k=\log_2(52)\times \frac{8}{7} + \gamma \xi\upsilon
%\end{equation}

%Notation 

%In (\ref{eq:hadi}), kd;jfsdl

%\begin{tabular}{|c|c|}
%	\hline  &  \\ 
%	\hline f & ew \\ 
%	\hline 54 & 545 \\ 
%	\hline 
%\end{tabular} 


==> Sections/Proof_lemma1.tex <==
Here, we prove Lemma \ref{lem:parityLRC}.
In an optimal LRC if there is less than $\frac{n}{r+1}$ local groups, at least in one local group more than $r+1$ blocks are get involved leads to the locality more than $r$. Hence at least $\frac{n}{r+1}$ local parity blocks are required and we have
\begin{multline*}
~~~~~~~~n-k \geq \frac{n}{r+1}\Rightarrow
k\le \frac{nr}{r+1}\Rightarrow
\Big\lceil\frac{k}{r}\Big\rceil \le \frac{n}{r+1}\Rightarrow~~~~~~~~\\
n-k-\Big\lceil\frac{k}{r}\Big\rceil+2 \ge n-k-\frac{n}{r+1}+2.~~~~~~~~
\end{multline*}
For an optimal LRC $d=n-k-\lceil\frac{k}{r}\rceil+2$, hence,
\begin{equation}\label{dgreaterthan}
d\ge n-k-\frac{n}{r+1}+2
\end{equation}
For the global parity blocks in a optimal LRC from (\ref{eq:minimumdistancebound}), we have
\begin{multline*}\label{eq:parityblocks} 
~~~~~~~~d = n - k - \Big\lceil\frac{k}{r}\Big\rceil + 2 \le n - k(1+\frac{1}{r}) + 2\Rightarrow\\
k \le n(1-\frac{1}{r+1}) - (d-2)(1-\frac{1}{r+1})\Rightarrow \\
n-k-\frac{n}{r+1} \ge d-2-\frac{d-2}{r+1}.~~~~~~~~~~~~~
\end{multline*}
Note that $(r+1)\mid n$. Hence, $n-k-\frac{n}{r+1}$ is an integer, and consequently
\begin{multline*}
~~~~~~~~~~~~n-k-\frac{n}{r+1}\ge \Big\lceil d-2-\frac{d-2}{r+1}\Big\rceil=\\
d-2+\Big\lceil-\frac{d-2}{r+1}\Big\rceil =d-2-\Big\lfloor\frac{d-2}{r+1}\Big\rfloor.~~~~~~~~
\end{multline*}
According to the assumption, $\frac{d-2}{r+1}< 1$. Hence, for an optimal LRC, we have
\begin{equation}\label{dlowerthan}
n-k-\frac{n}{r+1} \ge d-2.
\end{equation} 
Now, by considering (\ref{dgreaterthan}) and (\ref{dlowerthan}) we have:
\begin{equation*}
n-k-\frac{n}{r+1} = d-2.
\end{equation*} 
Note that among the total $n-k$ parity blocks, at least $\frac{n}{r+1}$ parity blocks are local. Hence, the remaining $n-k-\frac{n}{r+1}=d-2$ parity blocks are global.




==> Sections/Proof_rate.tex <==
Here, we prove Proposition \ref{prop:rate}.
From (\ref{eq:minimumdistancebound}), we have
\begin{multline*}
~~~~~~~~~d\le n-k-\Big\lceil \frac{k}{r} \Big\rceil+2 \le n-k-\frac{k}{r}+2
\\ \Rightarrow r\ge\frac{k}{n-k-d+2} ~~~~~~~~~~~~~~~~~~~~~~
\end{multline*}
Observe that if $d<\frac{k}{n-k-d+2}+3$, then $d<r+3$. We have
\begin{equation*}
d-3<\frac{k}{n-k-d+2}
\end{equation*} 
\begin{equation}\label{quadraticeq}
\Leftrightarrow d^2 -(n-k+5)d+(3n-2k+6)> 0
\end{equation}
Note that if the minimum of (\ref{quadraticeq}) is positive, (\ref{quadraticeq}) is always true. 
The minimum of this equation is achieved at $d=\frac{n-k+5}{2}$. We have  
\begin{multline*}
\Leftrightarrow \frac{(n-k+5)^2}{4}-\frac{(n-k+5)^2}{2}+(3n-2k+6)> 0
%\\ \Leftrightarrow \frac{(n-k+5)^2}{4}\le 3n-2k+6
\\ \Leftrightarrow n^2 - 2(k+1)n + (k-1)^2< 0
%\\ \Leftrightarrow k+1-2\sqrt{k} \le n \le k+1+2\sqrt{k}
\\ \Leftrightarrow (\sqrt{k}-1)^2 < n < (\sqrt{k}+1)^2
\\ \Leftrightarrow (\sqrt{R} - \frac{1}{\sqrt{n}})^2 < 1 < (\sqrt{R} + \frac{1}{\sqrt{n}})^2  
%\\ \Leftrightarrow 1-\frac{1}{\sqrt{n}} \le \sqrt{R} \le 1+\frac{1}{\sqrt{n}} 
\\ \Leftrightarrow R> (1-\frac{1}{\sqrt{n}})^2,~~~~~~~~~~~~~~~~~~~~~
\end{multline*} 
which concludes the proof.

==> Sections/mind.tex <==
Here, we prove Proposition \ref{prop:min_d}.
For an $(n,k)$ erasure code with Tanner graph $\mathcal{T}$, if any $\phi$ variable nodes are connected to $\phi$ distinct check nodes, where $\phi \in [d-1]$, then any $\phi$ variable nodes can be recovered using equations associated with the distinct check nodes.
This implies that the code can recover up to any $d-1$ failures and therefore, it has minimum distance $d$.

In our proposed LRCs, every information nodes is connected to at least $(d-2-\lfloor\frac{d-2}{r+1}\rfloor-(\lambda-\lfloor\frac{d-2}{r+1}\rfloor)+\lambda)+1=d-1$ distinct check nodes, where $\lambda=\lceil\frac{d-2-\lfloor\frac{d-2}{r+1}\rfloor}{r}\rceil$. 
Also, each of the $n-k$ parity nodes is connected to exactly one distinct check node. 
Hence, any $d-1$ variable nodes are connected to at least $d-1$ distinct check nodes and our proposed code has minimum distance $d$.
%Now, we show that any $\phi=d-1$ variable nodes are connected to $d-1$ distinct check nodes which concludes the proof.   
%
%For $\phi= d-1$, the worst case is when all $d-1$ variable nodes are in the same local group because otherwise, they have connection to at least $(d-2)+1=d-1$ check nodes.
%Observe that if $d-1$ variable nodes are in the last local group, they are connected to $d-1$ distinct check nodes. 
%For the case that $d-1$ variable nodes are not in the last local group, we show by contradiction that any $d-1$ variable node is covered by $d-1$ distinct check nodes.
%
%Assuming that all $d-1$ variable nodes are chosen from one of the first $n-k-d+1$ local groups, by contradiction, we assume that $d-1$ variable nodes are connected to one local and $d-3$ global check nodes. 
%In other words, there is a global check node which is not connected to $d-1$ variable nodes in a local group.  
%This contradicts the assumption that each global check node in our proposed LRCs does not cover at most $d-2$ variable nodes.
%

